Resource Aware Clustering for Tackling the Heterogeneity of Participants in Federated Learning

Federated Learning is a training framework that enables multiple participants to collaboratively train a shared model while preserving data privacy and minimizing communication overhead. The heterogeneity of devices and networking resources of the participants delay the training and aggregation in federated learning. This paper proposes a federated learning approach to manoeuvre the heterogeneity among the participants using resource aware clustering. The approach begins with the server gathering information about the devices and networking resources of participants, after which resource aware clustering is performed to determine the optimal number of clusters using Dunn Indices. The mechanism of participant assignment is then introduced, and the expression of communication rounds required for model convergence in each cluster is mathematically derived. Furthermore, a master-slave technique is introduced to improve the performance of the lightweight models in the clusters using knowledge distillation. Finally, experimental evaluations are conducted to verify the feasibility and effectiveness of the approach and to compare it with state-of-the-art techniques.

==> 1/CIFAR-10/1_ <==
set terminal epslatex 'phv,bx';
set output '1.tex'; 
set size 0.8,0.8;
set xlabel '\Large{\textbf{Length of MTS (100 - Earliness) (\%)}}' offset 1;
set ylabel '\Large{\textbf{Accuracy (\%)}}' offset 1;
set pointsize 0;
set ytics 0,10,100
#set xtics 0,10,100 

set key left Left box 3

set object 1 ellipse center 88,72 size 30, 10 angle 40 front fc rgb"green" behind fs solid 0.5 lw 1
#set label 'accuracy' at 35,90;
#set label '$(74 \mp 7.5)\%$' at 35,82;


plot [0:100][0:110] 'final_out_d' using 1:6 with linespoints lt 2 lc rgb "red" lw 5 title '\large \boldmath$\alpha=0.5$', 'final_out_d' using 1:5 with linespoints lt 1 lc rgb "blue" lw 5 title '\large \boldmath$\alpha=0.6$', 'final_out_d' using 1:4 with linespoints lt 4 lc rgb "black" lw 5 title '\large \boldmath$\alpha=0.7$', 'final_out_d' using 1:3 with linespoints lt 6 lc rgb "cyan" lw 5 title '\large \boldmath$\alpha=0.8$', 'final_out_d' using 1:2 with linespoints lt 5 lc rgb "magenta" lw 5 title '\large \boldmath$\alpha=0.9$'


==> 1/HAR/1_ <==
set terminal epslatex 'phv,bx';
set output '1.tex'; 
set size 0.8,0.8;
set xlabel '\Large{\textbf{Length of MTS (100 - Earliness) (\%)}}' offset 1;
set ylabel '\Large{\textbf{Accuracy (\%)}}' offset 1;
set pointsize 0;
set ytics 0,10,100
#set xtics 0,10,100 

set key left Left box 3

set object 1 ellipse center 88,72 size 30, 10 angle 40 front fc rgb"green" behind fs solid 0.5 lw 1
#set label 'accuracy' at 35,90;
#set label '$(74 \mp 7.5)\%$' at 35,82;


plot [0:100][0:110] 'final_out_d' using 1:6 with linespoints lt 2 lc rgb "red" lw 5 title '\large \boldmath$\alpha=0.5$', 'final_out_d' using 1:5 with linespoints lt 1 lc rgb "blue" lw 5 title '\large \boldmath$\alpha=0.6$', 'final_out_d' using 1:4 with linespoints lt 4 lc rgb "black" lw 5 title '\large \boldmath$\alpha=0.7$', 'final_out_d' using 1:3 with linespoints lt 6 lc rgb "cyan" lw 5 title '\large \boldmath$\alpha=0.8$', 'final_out_d' using 1:2 with linespoints lt 5 lc rgb "magenta" lw 5 title '\large \boldmath$\alpha=0.9$'


==> 1/SHL/1_ <==
set terminal epslatex 'phv,bx';
set output '1.tex'; 
set size 0.8,0.8;
set xlabel '\Large{\textbf{Length of MTS (100 - Earliness) (\%)}}' offset 1;
set ylabel '\Large{\textbf{Accuracy (\%)}}' offset 1;
set pointsize 0;
set ytics 0,10,100
#set xtics 0,10,100 

set key left Left box 3

set object 1 ellipse center 88,72 size 30, 10 angle 40 front fc rgb"green" behind fs solid 0.5 lw 1
#set label 'accuracy' at 35,90;
#set label '$(74 \mp 7.5)\%$' at 35,82;


plot [0:100][0:110] 'final_out_d' using 1:6 with linespoints lt 2 lc rgb "red" lw 5 title '\large \boldmath$\alpha=0.5$', 'final_out_d' using 1:5 with linespoints lt 1 lc rgb "blue" lw 5 title '\large \boldmath$\alpha=0.6$', 'final_out_d' using 1:4 with linespoints lt 4 lc rgb "black" lw 5 title '\large \boldmath$\alpha=0.7$', 'final_out_d' using 1:3 with linespoints lt 6 lc rgb "cyan" lw 5 title '\large \boldmath$\alpha=0.8$', 'final_out_d' using 1:2 with linespoints lt 5 lc rgb "magenta" lw 5 title '\large \boldmath$\alpha=0.9$'


==> 10/CIFAR-10/1_ <==
set terminal epslatex 'phv,bx';
set output '1.tex'; 
set size 0.8,0.8;
set xlabel '\Large{\textbf{Length of MTS (100 - Earliness) (\%)}}' offset 1;
set ylabel '\Large{\textbf{Accuracy (\%)}}' offset 1;
set pointsize 0;
set ytics 0,10,100
#set xtics 0,10,100 

set key left Left box 3

set object 1 ellipse center 88,72 size 30, 10 angle 40 front fc rgb"green" behind fs solid 0.5 lw 1
#set label 'accuracy' at 35,90;
#set label '$(74 \mp 7.5)\%$' at 35,82;


plot [0:100][0:110] 'final_out_d' using 1:6 with linespoints lt 2 lc rgb "red" lw 5 title '\large \boldmath$\alpha=0.5$', 'final_out_d' using 1:5 with linespoints lt 1 lc rgb "blue" lw 5 title '\large \boldmath$\alpha=0.6$', 'final_out_d' using 1:4 with linespoints lt 4 lc rgb "black" lw 5 title '\large \boldmath$\alpha=0.7$', 'final_out_d' using 1:3 with linespoints lt 6 lc rgb "cyan" lw 5 title '\large \boldmath$\alpha=0.8$', 'final_out_d' using 1:2 with linespoints lt 5 lc rgb "magenta" lw 5 title '\large \boldmath$\alpha=0.9$'


==> 10/CIFAR-10a/1_ <==
set terminal epslatex 'phv,bx';
set output '1.tex'; 
set size 0.8,0.8;
set xlabel '\Large{\textbf{Length of MTS (100 - Earliness) (\%)}}' offset 1;
set ylabel '\Large{\textbf{Accuracy (\%)}}' offset 1;
set pointsize 0;
set ytics 0,10,100
#set xtics 0,10,100 

set key left Left box 3

set object 1 ellipse center 88,72 size 30, 10 angle 40 front fc rgb"green" behind fs solid 0.5 lw 1
#set label 'accuracy' at 35,90;
#set label '$(74 \mp 7.5)\%$' at 35,82;


plot [0:100][0:110] 'final_out_d' using 1:6 with linespoints lt 2 lc rgb "red" lw 5 title '\large \boldmath$\alpha=0.5$', 'final_out_d' using 1:5 with linespoints lt 1 lc rgb "blue" lw 5 title '\large \boldmath$\alpha=0.6$', 'final_out_d' using 1:4 with linespoints lt 4 lc rgb "black" lw 5 title '\large \boldmath$\alpha=0.7$', 'final_out_d' using 1:3 with linespoints lt 6 lc rgb "cyan" lw 5 title '\large \boldmath$\alpha=0.8$', 'final_out_d' using 1:2 with linespoints lt 5 lc rgb "magenta" lw 5 title '\large \boldmath$\alpha=0.9$'


==> 10/HAR0/1_ <==
set terminal epslatex 'phv,bx';
set output '1.tex'; 
set size 0.8,0.8;
set xlabel '\Large{\textbf{Length of MTS (100 - Earliness) (\%)}}' offset 1;
set ylabel '\Large{\textbf{Accuracy (\%)}}' offset 1;
set pointsize 0;
set ytics 0,10,100
#set xtics 0,10,100 

set key left Left box 3

set object 1 ellipse center 88,72 size 30, 10 angle 40 front fc rgb"green" behind fs solid 0.5 lw 1
#set label 'accuracy' at 35,90;
#set label '$(74 \mp 7.5)\%$' at 35,82;


plot [0:100][0:110] 'final_out_d' using 1:6 with linespoints lt 2 lc rgb "red" lw 5 title '\large \boldmath$\alpha=0.5$', 'final_out_d' using 1:5 with linespoints lt 1 lc rgb "blue" lw 5 title '\large \boldmath$\alpha=0.6$', 'final_out_d' using 1:4 with linespoints lt 4 lc rgb "black" lw 5 title '\large \boldmath$\alpha=0.7$', 'final_out_d' using 1:3 with linespoints lt 6 lc rgb "cyan" lw 5 title '\large \boldmath$\alpha=0.8$', 'final_out_d' using 1:2 with linespoints lt 5 lc rgb "magenta" lw 5 title '\large \boldmath$\alpha=0.9$'


==> 10/HAR1/1_ <==
set terminal epslatex 'phv,bx';
set output '1.tex'; 
set size 0.8,0.8;
set xlabel '\Large{\textbf{Length of MTS (100 - Earliness) (\%)}}' offset 1;
set ylabel '\Large{\textbf{Accuracy (\%)}}' offset 1;
set pointsize 0;
set ytics 0,10,100
#set xtics 0,10,100 

set key left Left box 3

set object 1 ellipse center 88,72 size 30, 10 angle 40 front fc rgb"green" behind fs solid 0.5 lw 1
#set label 'accuracy' at 35,90;
#set label '$(74 \mp 7.5)\%$' at 35,82;


plot [0:100][0:110] 'final_out_d' using 1:6 with linespoints lt 2 lc rgb "red" lw 5 title '\large \boldmath$\alpha=0.5$', 'final_out_d' using 1:5 with linespoints lt 1 lc rgb "blue" lw 5 title '\large \boldmath$\alpha=0.6$', 'final_out_d' using 1:4 with linespoints lt 4 lc rgb "black" lw 5 title '\large \boldmath$\alpha=0.7$', 'final_out_d' using 1:3 with linespoints lt 6 lc rgb "cyan" lw 5 title '\large \boldmath$\alpha=0.8$', 'final_out_d' using 1:2 with linespoints lt 5 lc rgb "magenta" lw 5 title '\large \boldmath$\alpha=0.9$'


==> 11/1_ <==
set terminal epslatex 'phv,bx';
set output '1.tex'; 
set size 0.8,0.8;
set xlabel '\Large{\textbf{Length of MTS (100 - Earliness) (\%)}}' offset 1;
set ylabel '\Large{\textbf{Accuracy (\%)}}' offset 1;
set pointsize 0;
set ytics 0,10,100
#set xtics 0,10,100 

set key left Left box 3

set object 1 ellipse center 88,72 size 30, 10 angle 40 front fc rgb"green" behind fs solid 0.5 lw 1
#set label 'accuracy' at 35,90;
#set label '$(74 \mp 7.5)\%$' at 35,82;


plot [0:100][0:110] 'final_out_d' using 1:6 with linespoints lt 2 lc rgb "red" lw 5 title '\large \boldmath$\alpha=0.5$', 'final_out_d' using 1:5 with linespoints lt 1 lc rgb "blue" lw 5 title '\large \boldmath$\alpha=0.6$', 'final_out_d' using 1:4 with linespoints lt 4 lc rgb "black" lw 5 title '\large \boldmath$\alpha=0.7$', 'final_out_d' using 1:3 with linespoints lt 6 lc rgb "cyan" lw 5 title '\large \boldmath$\alpha=0.8$', 'final_out_d' using 1:2 with linespoints lt 5 lc rgb "magenta" lw 5 title '\large \boldmath$\alpha=0.9$'

